SIMD Lossy Compression for Scientific Data

Modern HPC applications produce increasingly large amounts of data, which limits the performance of current extreme-scale systems. Data reduction techniques, such as lossy compression, help to mitigate this issue by decreasing the size of data generated by these applications. SZ, a current state-of-the-art lossy compressor, is able to achieve high compression ratios, but the prediction/quantization methods used introduce dependencies which prevent parallelizing this step of the compression. Recent work proposes a parallel dual prediction/quantization algorithm for GPUs which removes these dependencies. However, some HPC systems and applications do not use GPUs, and could still benefit from the fine-grained parallelism of this method. Using the dual-quantization technique, we implement and optimize a SIMD vectorized CPU version of SZ, and create a heuristic for selecting the optimal block size and vector length. We also investigate the effect of non-zero block padding values to decrease the number of unpredictable values along compression block borders. We measure performance of vecSZ against an O3 optimized CPU version of SZ using dual-quantization, pSZ, as well as SZ-1.4. We evaluate our vectorized version, vecSZ, on the Intel Skylake and AMD Rome architectures using real-world scientific datasets. We find that applying alternative padding reduces the number of outliers by 100\% for some configurations. Our implementation also results in up to 32\% improvement in rate-distortion and up to 15$\times$ speedup over SZ-1.4, achieving a prediction and quantization bandwidth in excess of 3.4 GB/s.

==> sec/alg_dualquant.tex <==
% \small\sffamily
% \begin{algorithmic}[1] % The number tells where the line numbering should start
% \Statex {\color{B}$\bullet$\bfseries\sffamily\ archive (compression) procedure}
% \For{$\forall d\in D$ concurrently}
%     \State \makebox[1.25em][l]{$d^\circ$}%
%         \makebox[6em][l]{$\gets d/(2\!\times\!eb)$}%
%         \textcolor{B}{\sffamily\scshape\bfseries barrier} \Comment{\textsc{\textbf{pre}quantization}} %\Comment{remain FP representation}
%     \Statex \Comment{remain floating-point representation}
%     % \Statex \hspace{\algorithmicindent}\textcolor{gray}{\scshape explict barrier}
%     \State \makebox[1.25em][l]{$d$}%
%         \makebox[6em][l]{$\gets d^\circ$}%
%         \textcolor{B}{\sffamily\scshape\bfseries barrier} \Comment{memory reuse ($d\leftrightarrow d^\circ$)}
%     \State \makebox[1.25em][l]{$p^\circ$}$\gets\ell(d^\circ_\text{\scshape sr})$, $e^\circ \gets p^\circ\! - d^\circ$
%     \If{$e^\circ < $ \textsc{cap/2 (in-cap)} }   \Comment{\textsc{\textbf{post}quantization}}
%         \State $e^\circ_\text{D} \gets$ \textsc{cast\textless float2int\textgreater}$(e^\circ)$ %\Comment{\texttt{FP} to \texttt{INT} representation}
%     \Else
%         \State \textsc{outlier: }$e^\circ_\text{D} \gets 0$ and record the verbatim $x\gets d^\circ$
%     \EndIf
% \EndFor
% % \Statex
% \Statex {\color{B}$\bullet$\bfseries\sffamily\ extract (decompression) procedure}
% \For{$d^\bullet\in D^\bullet$ to reconstruct cascadingly}
%     \State $p^\bullet\gets\ell(d^\bullet_\text{\scshape sr})$
%     \State $d^\bullet\gets (p^\bullet + e^\circ_\text{D})\cdot (2\!\times\!eb)$ if \textsc{in-cap} else verbatim $x$
% \EndFor
% \end{algorithmic}

\iffalse
\begin{algorithmic}[1] % The number tells where the line numbering should start
\For{$\forall d\in D$ concurrently}
    \Comment{{\color{B}\fontfamily{ugq}\selectfont compression}}
    \State \makebox[1.25em][l]{$d^\circ$}%
        \makebox[6em][l]{$\gets d/(2\!\times\!eb)$}%
        % \textcolor{B}{\sffamily\scshape\bfseries barrier} 
        \Comment{(FP representation) \textsc{\textbf{pre}quant}} %\Comment{remain FP representation}
    % \Statex \Comment{remain floating-point representation}
    % \Statex \hspace{\algorithmicindent}\textcolor{gray}{\scshape explict barrier}
    \State \makebox[1.25em][l]{$d$}%
        \makebox[6em][l]{$\gets d^\circ$}%
        % \textcolor{B}{\sffamily\scshape\bfseries barrier} \Comment{memory reuse ($d\leftrightarrow d^\circ$)}
        \Comment{{\sffamily\bfseries\scshape barrier}}
    \State \makebox[1.25em][l]{$p^\circ$}$\gets\ell(d^\circ_\text{\scshape sr})$, $\delta^\circ \gets p^\circ\! - d^\circ$
    \If{$\delta^\circ < $ \textsc{cap/2 (in-cap)} }   \Comment{\textsc{\textbf{post}quant}}
        \State $\delta^\circ_\text{D} \gets$ \textsc{cast\textless float2int\textgreater}$(\delta^\circ)$ %\Comment{\texttt{FP} to \texttt{INT} representation}
    \Else
        \State \textsc{outlier: }$\delta^\circ_\text{D} \gets 0$ and record the verbatim $x\gets d^\circ$
    \EndIf
\EndFor
\Statex
\For{$d^\bullet\in D^\bullet$ to reconstruct cascadingly}
\Comment{{\color{B}\fontfamily{ugq}\selectfont decompression}}
    \State $p^\bullet\gets\ell(d^\bullet_\text{\scshape sr})$
    \State $d^\bullet\gets (p^\bullet + \delta^\circ_\text{D})\cdot (2\!\times\!eb)$ if \textsc{in-cap} else verbatim $x$
\EndFor
\end{algorithmic}
\fi






\begin{algorithm}[h]
\SetAlgoLined
\DontPrintSemicolon
\SetKwFunction{Compress}{compress}
\SetKwFunction{Decompress}{decompress}
\scriptsize
%\footnotesize
  \SetKwProg{Fn}{Function}{}{}
  \Fn{\Compress{}}{
  
    \For{$\forall d\in D$ concurrently} {
    %\Comment{{\color{B}\fontfamily{ugq}\selectfont compression}}

        $d^\circ\gets round( d/(2\!\times\!eb) )$%
        % \textcolor{B}{\sffamily\scshape\bfseries barrier} 
        \tcp*{\textbf{pre}-quant}\\ %\Comment{remain FP representation}
    % \Statex \Comment{remain floating-point representation}
    % \Statex \hspace{\algorithmicindent}\textcolor{gray}{\scshape explict barrier}
    %\makebox[1.25em][l]{$d$}%
    %    \makebox[6em][l]{$\gets d^\circ$
$d\gets d^\circ$%
        % \textcolor{B}{\sffamily\scshape\bfseries barrier} \Comment{memory reuse ($d\leftrightarrow d^\circ$)}
        \tcp*{{\sffamily\bfseries barrier}} \\
    %\makebox[1.25em][l]{$p^\circ$}$\gets\ell(d^\circ_\text{\scshape sr})$\\
    %$\delta^\circ \gets p^\circ\! - d^\circ$
    $p^\circ\gets\ell(d^\circ_\text{sr})$\\
    $\delta^\circ \gets p^\circ\! - d^\circ$
    
    
    
    \;
    
    \uIf(\hfill \tcp*[h]{\textbf{post}-quant}){$\delta^\circ < $ \textsc{cap/2 (in-cap)} } {  
        $\delta^\circ_\text{D} \gets$ \textsc{cast\textless float2int\textgreater}$(\delta^\circ)$\\ %\Comment{\texttt{FP} to \texttt{INT} representation}
        }
    \Else {
          \textsc{outlier: }$\delta^\circ_\text{D} \gets 0$ and record the verbatim $x\gets d^\circ$
    }
    }
}

 \Fn{\Decompress{}}{
  
    \For{$d^\bullet\in D^\bullet$ to reconstruct cascadingly} {
%\Comment{{\color{B}\fontfamily{ugq}\selectfont decompression}}
    $p^\bullet\gets\ell(d^\bullet_\text{sr})$ \\
    $d^\bullet\gets (p^\bullet + \delta^\circ_\text{D})\cdot (2\times eb)$ if \textsc{in-cap} else verbatim $x$
    
}
}



 \caption{\label{algo:dual-quant} vecSZ compression and decompression.}
\end{algorithm}

==> sec/alg_orig_sz.tex <==
% \small\sffamily
% \begin{algorithmic}[1] % The number tells where the line numbering should start
% \Statex {\color{B}$\bullet$\bfseries\sffamily\ archive (compression) procedure}
% \For{$d\in D$}
%     \State $p^\circ \gets\ell(d_\textsc{\scshape sr})$, $e^\circ \gets p^\circ\! - d$
%     \If{$e^\circ/eb < $ \textsc{cap (in-cap)} }   \Comment{quantization}
%         \State $e^\circ_\text{D} \gets$ \textsc{integerize}$(e^\circ/(2\!\times\!eb))$
%         \State \textsc{rehearsal} $\gets p^\circ + 2\cdot e^\circ_\text{D}\cdot eb$
%         \State \textsc{watchdog}($\text{\scshape rehearsal} - d < eb$, fallback: \textsc{outlier})
%     \Else
%         \State \textsc{outlier: }$e^\circ_\text{D} \gets 0$ and record the verbatim $x\gets d$
%     \EndIf
%     \State $d\gets$ \textsc{rehearsal} or $x$ accordingly
%     \Comment{incurs \textsc{\bfseries raw}}
% \EndFor
% % \Statex
% \Statex {\color{B}$\bullet$\bfseries\sffamily\ extract (decompression) procedure}
% \For{$d^\bullet\in D^\bullet$ to reconstruct cascadingly}
%     \State $p^\bullet\gets\ell(d^\bullet_\text{\scshape sr})$
%     \State $d^\bullet\gets p^\bullet + 2\cdot e^\circ_\text{D}\cdot eb$ if \textsc{in-cap} else verbatim $x$
% \EndFor
% \end{algorithmic}


\iffalse
%\small\sffamily
\begin{algorithmic}[1] % The number tells where the line numbering should start
% \Statex {\color{B}$\bullet$\bfseries\sffamily\ archive (compression) procedure}
\For{$d\in D$}
    %\Comment{{\color{B}\fontfamily{ugq}\selectfont compression}}
    $p^\circ \gets\ell(d_\textsc{\scshape sr})$ \\
    $e^\circ \gets p^\circ\! - d$ \\ 
    \If(\tcp*[h]{quantization}){$e^\circ/eb < $ \textsc{cap (in-cap)} }
        $e^\circ_\text{D} \gets$ \\ \textsc{integerize}$(e^\circ/(2\!\times\!eb))$ \\
        \State \textsc{rehearsal} $\gets p^\circ + 2\cdot \\ e^\circ_\text{D}\cdot eb$ \\
        \textsc{watchdog}($\text{\scshape rehearsal} - d < eb$, fallback: \textsc{outlier})
    \Else
        \State \textsc{outlier: }$e^\circ_\text{D} \gets 0$ and record the verbatim $x\gets d$
    \EndIf
   
\EndFor
\Statex
\For{$d^\bullet\in D^\bullet$ to reconstruct cascadingly}
\Comment{{\color{B}\fontfamily{ugq}\selectfont decompression}}
    \State $p^\bullet\gets\ell(d^\bullet_\text{\scshape sr})$
    \State $d^\bullet\gets p^\bullet + 2\cdot e^\circ_\text{D}\cdot eb$ if \textsc{in-cap} else verbatim $x$
\EndFor
\end{algorithmic}
\fi


\begin{algorithm}[h]
\SetAlgoLined
\DontPrintSemicolon
\SetKwFunction{Compress}{compress}
\SetKwFunction{Decompress}{decompress}
%\footnotesize
\scriptsize
  \SetKwProg{Fn}{Function}{}{}
  \Fn{\Compress{}}{
  
    \For{$d\in D$} {
    %\tcp*{{\color{B}\fontfamily{ugq}\selectfont compression}}\\
    $p^\circ \gets\ell(d_\textsc{\scshape sr})$\\
    %p^\circ \gets\ell(d)$\\
    $e^\circ \gets p^\circ\! - d$\\
    \;

    \uIf(\hfill\tcp*[h]{\textbf{quantization}}){$e^\circ/eb < $ \textsc{cap (in-cap)} }{  
        $e^{\circ}_{\text{D}} \gets \textsc{integerize} (e^{\circ} / (2 \times eb))$\\
        \textsc{reconstructed} $\gets p^\circ + 2\cdot e^\circ_\text{D}\cdot eb$ \\
        \textsc{watchdog}($\textsc{reconstructed} - d < eb$, fallback: \textsc{outlier})\\
        
        }
    \Else {
         \textsc{outlier: }$e^\circ_\text{D} \gets 0$ and record the verbatim $x\gets d$\\
    }
        \;
    $d\gets$ \text{\textsc{reconstructed}} or $x$ accordingly 
    \tcp*{incurs \textbf{ raw}}
}
}
 \Fn{\Decompress{}}{
  
    \For{$d^\bullet\in D^\bullet$ to reconstruct cascadingly} {
%\Comment{{\color{B}\fontfamily{ugq}\selectfont decompression}}
    $p^\bullet\gets\ell(d^\bullet_\text{sr})$ \\
    $d^\bullet\gets p^\bullet + 2\cdot e^\circ_\text{D}\cdot eb$ if \text{\textsc{in-cap}} else verbatim $x$
    
}
}

 \caption{\label{algo:original_sz} SZ-1.4 compression and decompression.}
\end{algorithm}

==> sec/related.tex <==
\section{Related Work} \label{sec:related}


Lossy compression algorithms have seen rapid advancements in recent years to combat issues related to data movement and storage on HPC systems. Two of the most well known are SZ~\cite{SZ} and ZFP~\cite{ZFP}. Recent versions of these algorithms improve their single threaded compression/decompression bandwidth and compression ratio~\cite{SZ_Paper2, SZ_2.0, SZ_auto}. For additional improvements, these algorithms have been ported to a variety of accelerators such as GPUs~\cite{cusz} and FPGAs~\cite{ZFP_V, waveSZ, GhostSZ}. Recent versions of SZ add additional methods to bound the compression error such as point-wise relative~\cite{SZ_PW_REL} and PSNR~\cite{SZ_PSNR}. To efficiently configure compression algorithms, FRaZ~\cite{underwood2020fraz} enables general lossy compression algorithms to compress data to a target size by solving an optimization problem for selecting the compressor's error bound. 

Talk about vectorization optimization
